Learning to Organize Knowledge and Answer Questions with N-Gram Machines

Though deep neural networks have great success in natural language processing, they are limited at more knowledge intensive AI tasks, such as open-domain Question Answering (QA). Existing end-to-end deep QA models need to process the entire text after observing the question, and therefore their complexity in responding a question is linear in the text size. This is prohibitive for practical tasks such as QA from Wikipedia, a novel, or the Web. We propose to solve this scalability issue by using symbolic meaning representations, which can be indexed and retrieved efficiently with complexity that is independent of the text size. We apply our approach, called the N-Gram Machine (NGM), to three representative tasks. First as proof-of-concept, we demonstrate that NGM successfully solves the bAbI tasks of synthetic text. Second, we show that NGM scales to large corpus by experimenting on "life-long bAbI", a special version of bAbI that contains millions of sentences. Lastly on the WikiMovies dataset, we use NGM to induce latent structure (i.e. schema) and answer questions from natural language Wikipedia text, with only QA pairs as weak supervision.

==> discussion.tex <==
\section{Discussion}

%\paragraph{Evaluation}
Though the performance on bAbI tasks is satisfactory, it does not provide a realistic evaluation of how effective NGM is on natural languages -- bAbI was originally created from a small set of rules and primitives. 
However, we have presented a novel framework, and points to a new direction of how a long lasting problem in search might be solved.
%
A logical next step is to apply NGM to tasks with more natural languages.

For NGM to be effective, it depends on 1) whether the representation is expressive enough for useful natural language, and 2) whether the optimization can find an optimal representation with good sample complexity.
%
The expressiveness is determined by both the knowledge storage and programs.
When $n$ equals three, the n-grams have the same expressive power as the RDF triples used in Freebase~\cite{bollacker2008freebase}.
The \texttt{Hop} and related functions are  equivalent to traversal on the graph specified by the tri-grams.
%
Although we focus on extractive QA in this work, it will be easy to support broader semantics by adding more functions such as count and summation.
%
In NGM, there is no predefined distinction between entities and predicates -- e.g., the symbol ``father'' can perform either like a predicate or an entity, which removes the need to make such hard decisions manually.
%

A very expressive formalism might introduce a too big search space, therefore trade offs need to be made between expressiveness and learnability.
For example, though the most basic semantic units in NGM (i.e. symbols) can be any discrete objects, currently we restrict them to pre-tokenized words.
This choice is reasonable for the bAbI tasks, but might be too restricted in future applications.
%For example, should ``airplane designer'' be one symbol or two symbols?
%This should probably depend on 1) what questions are asked, and 2) how the functions extract answers, i.e. whether \texttt{Hop} extracts one symbol or a span of symbols.

==> more-related.tex <==
\subsection{More Related Work}
%The reminder of 
In this section analyzes why existing text understanding technologies are fundamentally limited and draws connections of our proposed solution to psychology and neuroscience.

\subsubsection{Current Practice in Text Understanding }
In recent years, several large-scale knowledge bases (KBs) have been constructed,  such as YAGO~\cite{suchanek2007yago}, Freebase~\cite{bollacker2008freebase}, NELL~\cite{mitchell2015nell}, Google Knowledge Graph~\cite{singhal2012kg}, Microsoft Satori~\cite{qian2013satori}, and others.
However, all of them suffer from a completeness problem \cite{dong2014vault} relative to large text corpora, which  stems from an inability to convert \emph{arbitrary} text to graph structures, and accurately answering questions from these structures.
There are two core issues in this difficulty:

\paragraph{The schema (or representation) problem} 
Traditional text extraction approaches need some fixed and finite target schema~\cite{riedel2013schema}.
For example, the definition of marriage\footnote{\url{https://en.wikipedia.org/wiki/Marriage}} is very complex and includes a whole spectrum of concepts, such as common-law marriage, civil union, putative marriage, handfasting, nikah mut'ah, and so on. 
It is prohibitively expensive to have experts to clearly define all these differences in advance, and annotate enough utterances from which they are expressed.
However, given a particular context, many of this distinctions might be irrelevant.
For example when a person say ``I just married Lisa.'' and then ask ``Who is my wife?'', a system should be able to respond correctly, without first learning about all types of marriage.
A desirable solution should induce schema automatically from the corpus such that knowledge encoded with this schema can help downstream tasks such as QA.

\paragraph{The end-to-end training (or inference) problem} 
The state-of-the-art approaches break down QA solutions into independent components, and manually annotate training examples for each of them.
Typical components include schema definition~\cite{mitchell2015nell,bollacker2008freebase}, relation extraction~\cite{mintz2009distant}, entity resolution~\cite{singla2006entity}, and semantic parsing~\cite{berant2013semantic,liang2017nsm}. 
However, these components need to work together and depend on each other. 
For example, the meaning of text expressions (e.g., ``father of IBM'', ``father of Adam Smith'', ``father of electricity'') depend on entity types. 
The type information, however, depends on the entity resolution decisions, and the content of the knowledge base (KB). The content of the KBs, if populated from text, will in return depend on the meaning of text expressions.
Existing systems~\cite{dong2014vault,berant2013semantic} leverage human annotation and supervised training for each component separately, which create consistency issues, and preclude directly optimizing the performance of the QA task.
A desirable solution should use few human annotations of intermediate steps, and rely on end-to-end training to directly optimize the QA quality.

\subsubsection{Text Understanding with Deep Neural Nets}
More recently there has been a lot of progress in applying deep neural networks (DNNs) to text understanding~\cite{mikolov2013composition, weston2014memory, neelakantan2015neural, graves2016hybrid, miller2016key}. 
The key ingredient to these solutions is embedding text expressions into a latent \emph{continuous} space. 
This removes the need to manually define a schema, while the vectors still allow complex inference and reasoning.
Continuous representations greatly simplified the system design of QA systems, and enabled end-to-end training, which directly optimizes the QA quality.
%
However, a key issue that prevents these models from being applied to many applications is scalability.
After receiving a question, all text in a corpus need to be analyzed by the model.
Therefore it leads to at least $O(n)$ complexity, where $n$ is the text size.
Approaches which rely on a search subroutine (e.g., DrQA~\cite{chen2017reading}) lose the benefit of end-to-end training, and are limited by the quality of the retrieval stage, which itself is difficult.

\subsubsection{Relationship to Neuroscience}
\label{sec:neuroscience}
Previous studies~\cite{wickman2012brain,bartol2015bound} of hippocampus suggests that human memory capacity may be somewhere between 10 terabytes and 100 terabytes.
This huge capacity is very advantageous for humans' survival, yet puts human brain in the same situation of a commercial search engine~\cite{brin1998search} -- facing the task of organizing vast amounts of information in a form which support fast retrieval and inference.
Good representations can only be learned gradually with a lot of computations, and the aggregated statistics of a lot of experiences.

Our model (Figure~\ref{fig:model}) resembles the complementary learning theory~\cite{mcclelland1995cls, oreilly2014cls, kumaran2016cls}, which hypothesizes that intelligent agents possess two learning systems, instantiated in mammals in the  hippocampus and neocortex.
%
The first quickly learns the specifics of individual experiences, which is essential for rapid adaptations~\cite{garcia1966},
while the second gradually acquires good knowledge representations for scalable and effective inference. 
The stories in training examples (episodic memories) and knowledge store (keys to episodic memories) represents the fast learning neurons, while the sequence to sequence (seq2seq) DNN models represent the slow learning neurons (semantic memory).
The DNN training procedure, which goes over the past experience (stories) over and over again, resembles the ``replay'' of hippocampal memories that allows goal-dependent weighting of experience statistics~\cite{kumaran2016cls}.

The auto-encoder (Section~\ref{sec:search}) is related to autoassociative memory, such as the CA3 recurrent collateral system in the hipposcampus~\cite{rolls2016cerebral}.
Similar to autoassociative networks, such as the Hopfield network~\cite{hopfield1982neural}, that can recall the memory when provided with a fragment of it, the knowledge decoder in our framework learns to recover the full sentence given noisy partial observations of it, i.e. all knowledge tuples of length $N$ that consist of only words from the text.
It also embodies \cite{tulving1983elements}'s hypothesis that the episodic memory is not just stored as engrams (n-grams), but also in the procedure (seq2seq), which reconstructs experience from the engrams.

The structure tweak procedure (Section~\ref{sec:search}) in our model is critical for its success, and resemblances the reconstructive (or generative) memory theory~\cite{piaget1977development,block1982development}, which
hypothesizes that by employing reconstructive processes, individuals supplement other aspects of available personal knowledge into the gaps found in episodic memory in order to provide a fuller and more coherent version. 
Our analysis of the QA task showed that at knowledge encoding stage information is often encoded without  understanding how it is going to be used.
So it might be encoded in an inconsistent way.
At the later QA stage an inference procedure tries to derive the expected answer by putting together several pieces of information, and fails due to inconsistency.
Only at that time can a hypothesis  be formed to retrospectively correct the inconsistency in memory.
These ``tweaks'' in memory later participate in training the knowledge encoder in the form of experience replay.

Our choice of using n-grams as the unit of knowledge storage is partially motivated by the Adaptive Resonance Theory (ART)~\cite{carpenter1997art,carpenter2003art, wang2012neuralmodeling}, which models each piece of human episodic memory as a set of symbols, each representing one aspect of the experience such as location, color, object etc.
